The morphology of star-forming gas and its alignment with galaxies and dark matter haloes in the EAGLE simulations

We present measurements of the morphology of star-forming gas in galaxies from the EAGLE simulations, and its alignment relative to stars and dark matter (DM). Imaging of such gas in the radio continuum enables weak lensing experiments that complement traditional optical approaches. Star-forming gas is typically more flattened than its associated stars and DM, particularly for present-day subhaloes of total mass $\sim$$10^{ 12-12.5} \mathrm{M_{ \odot}}$, which preferentially host star-forming galaxies with rotationally-supported stellar discs. Such systems have oblate, spheroidal star-forming gas distributions, but in both less- and more-massive subhaloes the distributions tend to be prolate, and its morphology correlates positively and significantly with that of its host galaxy's stars, both in terms of sphericity and triaxiality. The minor axis of star-forming gas most commonly aligns with the minor axis of its host subhalo's DM, but often aligns more closely with one of the other two principal axes of the DM distribution in prolate subhaloes. Star-forming gas aligns with DM less strongly than is the case for stars, but its morphological minor axis aligns closely with its kinematic axis, affording a route to observational identification of the unsheared morphological axis. The projected ellipticities of star-forming gas in EAGLE are consistent with shapes inferred from high-fidelity radio continuum images, and they exhibit greater shape noise than is the case for images of the stars, owing to the greater characteristic flattening of star-forming gas with respect to stars.

==> Hill et al. - Morphology & Internal Alignment v2/rcrain_shortcuts.tex <==
% Units                             
\newcommand{\cm}{{\rm cm}}
\newcommand{\g}                         {{\rm g}}
\newcommand{\yr}                         {\,{\rm yr}}
\newcommand{\peryr}                    {\,{\rm yr}^{-1}}
\newcommand{\Myr}                      {\,{\rm Myr}}
\newcommand{\perMyr}                 {\,{\rm Myr}^{-1}}
\newcommand{\Gyr}                      {\,{\rm Gyr}}
\newcommand{\perGyr}                 {\,{\rm Gyr}^{-1}}
\newcommand{\pc}                        {\,{\rm pc}}
\newcommand{\kpc}                      {\,{\rm kpc}}
\newcommand{\Mpc}                      {\,{\rm Mpc}}
\newcommand{\ppc}                        {\,{\rm ppc}}
\newcommand{\pkpc}                      {\,{\rm{pkpc}}}
\newcommand{\pMpc}                      {\,{\rm pMpc}}
\newcommand{\cpc}                        {\,{\rm cpc}}
\newcommand{\ckpc}                      {\,{\rm ckpc}}
\newcommand{\cMpc}                      {\,{\rm cMpc}}
\newcommand{\Msun}                    {\,{\rm M}_\odot}
\newcommand{\perMsun}                  {\,{\rm M}_\odot^{-1}}
\newcommand{\Msunsqpc}                    {\,{\rm M}_\odot\,{\rm pc}^{-2}}
\newcommand{\Msunyrsqkpc}                  {\,{\rm M}_\odot\,{\rm yr}^{-1}\,{\rm kpc}^{-2}}
\newcommand{\Msunyr}                 {\,{\rm M}_\odot\,{\rm yr}^{-1}}
\newcommand{\MsunyrMpccubed} {\,{\rm M}_\odot\,{\rm yr}^{-1}\,{\rm Mpc}^{-3}}
\newcommand{\hkpc}                     {\,h\,{\rm kpc}}
\newcommand{\hMpc}                     {\,h\,{\rm Mpc}}
\newcommand{\hckpc}                     {\,h\,{\rm ckpc}}
\newcommand{\hcMpc}                     {\,h\,{\rm cMpc}}
\newcommand{\hinvkpc}                  {\,h^{-1}\,{\rm kpc}}
\newcommand{\hinvMpc}                  {\,h^{-1}\,{\rm Mpc}}
\newcommand{\hinvckpc}                  {\,h^{-1}\,{\rm ckpc}}
\newcommand{\hinvcMpc}                  {\,h^{-1}\,{\rm cMpc}}
\newcommand{\hMsun}                  {\,h^{-1}\,{\rm M}_\odot}
\newcommand{\kms}                      {\,\,{\rm km}\,\,{\rm s}^{-1}}
\newcommand{\cmsquared}              {{\rm cm}^{-2}}
\newcommand{\cmcubed}              {{\rm cm}^{-3}}
\newcommand{\Zsun}                     {\,{\rm Z}_\odot}
\newcommand{\erg}                       {\,{\rm erg}}
\newcommand{\ergs}                     {\,{\rm erg}\,\,{\rm s}^{-1}}
\newcommand{\ergscm}                 {\,{\rm erg}\,{\rm s}^{-1}\,{\rm cm}^{-2}}
\newcommand{\ergperg}                 {\,{\rm erg}\,{\rm g}^{-1}}
\newcommand{\K}                          {\,{\rm K}}
\newcommand{\eV}                      {\,{\rm eV}}
\newcommand{\keV}                      {\,{\rm keV}}
\newcommand{\LKsun}                  {\,{\rm L}_{{\rm K},\odot}}
\newcommand{\ergsecHz}             {\,{\rm erg}\,\,{\rm s}^{-1}\,{\rm Hz}^{-1}}
\newcommand{\Msunyrkpcsq} {\,{\rm M}_\odot\,{\rm yr}^{-1}\,{\rm kpc}^{-2}}
\newcommand{\nHtc}{n_{{\rm H},t_{\rm c}}}
\newcommand{\PresUnit}{\,{\rm K\,cm}^{-3}}
\newcommand{\dex}              {{\rm dex}}

% Simulation related shortcuts
\newcommand{\gadget}         {\textsc{gadget3}}
\newcommand{\subfind}        {\textsc{subfind}}
\newcommand{\cloudy}         {\textsc{cloudy}}
\newcommand{\galexev}        {\textsc{galaxev}}
\newcommand{\apec}           {\textsc{apec}}
\newcommand{\cmbfast}        {\textsc{cmbfast}}
\newcommand{\camb}           {\textsc{camb}}
\newcommand{\panphasia}       {\textsc{panphasia}}
\newcommand{\gimic}          {\textsc{gimic}}
\newcommand{\sz}             {\hbox{$0\sigma$}}
\renewcommand{\sp}           {\hbox{$+1\sigma$}}
\newcommand{\spp}            {\hbox{$+2\sigma$}}
\newcommand{\sm}             {\hbox{$-1\sigma$}}
\newcommand{\smm}            {\hbox{$-2\sigma$}}
\newcommand{\owls}           {\textsc{owls}}
\newcommand{\eagle}          {\textsc{eagle}}
\newcommand{\snconstnoagn}   {\textsc{SNconst-noagn}}
\newcommand{\snconst}        {\textsc{SNconst}}
\newcommand{\snsigma}        {\textsc{SN$\sigma$}}
\newcommand{\snZ}            {\textsc{SNZ}}
\newcommand{\snZrho}         {\textsc{SNZ$\rho$}}
\newcommand{\Reff}            {\textsc{Ref}}
\newcommand{\weak}           {\textsc{WeakSN}}
\newcommand{\strong}         {\textsc{StrongSN}}


%Misc 
\newcommand{\skirt}         {\textsc{SKIRT}}
\newcommand{\treesph}         {\textsc{TreeSPH}}
\newcommand{\omegam}        {$\Omega_{\rm m}$}
\newcommand{\omegalam}        {$\Omega_{\Lambda}$}
\newcommand{\omegab}        {$\Omega_{\rm b}$}
\newcommand{\omegastar}    {$\Omega_\star$}
\newcommand{\osix}              {O\textsc{vi}}
\newcommand{\oseven}          {O\textsc{vii}}
\newcommand{\cfour}             {C\textsc{iv}}
\newcommand{\einstein}             {\textit{Einstein}}
\newcommand{\rosat}             {\textit{ROSAT}}
\newcommand{\asca}             {\textit{ASCA}}
\newcommand{\chandra}         {\textit{Chandra}}
\newcommand{\xmm}             {\textit{XMM-Newton}}
\newcommand{\ixo}             {\textit{IXO}}
\newcommand{\iras}             {\textit{IRAS}}
\newcommand{\galex}             {\textit{GALEX}}
\newcommand{\twomass}       {\textsc{2Mass}}
\newcommand{\ipac}              {\textsc{Ipac}}
\newcommand{\mast}             {\textsc{Mast}}
\newcommand{\lstar}             {$L_\star$}
\newcommand{\lcdm}             {$\Lambda$CDM}

\newcommand{\Hub}               {$H_0$}
\newcommand{\sigeight}          {$\sigma_8$}
\newcommand{\ns}          {$n_{\rm s}$}

\newcommand{\sfr}                {\dot{M}_\star}
\newcommand{\lx}                 {L_{\rm X}}
\newcommand{\lk}                 {L_{\rm K}}
\newcommand{\lb}                 {L_{\rm B}}
\newcommand{\Tx}                {T_{\rm X}}
\newcommand{\kTx}              {k_{\rm B}T_{\rm X}}
\newcommand{\vrot}              {v_{\rm rot}}
\newcommand{\mstar}           {M_{\star}}
\newcommand{\mvir}              {M_{\rm vir}}
\newcommand{\lxlk}              {L_{\rm X} - L_{\rm K}}
\newcommand{\lxlb}              {L_{\rm X} - L_{\rm B}}
\newcommand{\lxvrot}           {L_{\rm X} - v_{\rm rot}}
\newcommand{\lxsfr}             {L_{\rm X} - \dot{M}_\star}
\newcommand{\lxTx}              {L_{\rm X} - T_{\rm X}}
\newcommand{\lxmvir}          {L_{\rm X} - M_{\rm vir}}
\newcommand{\lkmvir}          {L_{\rm K} - M_{\rm vir}}
\newcommand{\ZFe}               {Z_{\rm Fe}}
\newcommand{\ZFesun}       {{\rm Z}_{\rm Fe,\odot}}
\newcommand{\nH}           {n_{\rm H}}
\newcommand{\tcool}          {t_{\rm cool}}
\newcommand{\tdyn}          {t_{\rm dyn}}

\newcommand{\itleft}       {\textit{left}}
\newcommand{\itright}      {\textit{right}}
\newcommand{\itLeft}       {\textit{Left}}
\newcommand{\itRight}      {\textit{Right}}
\newcommand{\HI}         {H\textsc{I}}
\newcommand{\HII}         {H\textsc{II}}
\newcommand{\Hmol}       {${\rm H}_2$}

